Self-Healing Robust Neural Networks via Closed-Loop Control

Despite the wide applications of neural networks, there have been increasing concerns about their vulnerability issue. While numerous attack and defense techniques have been developed, this work investigates the robustness issue from a new angle: can we design a self-healing neural network that can automatically detect and fix the vulnerability issue by itself? A typical self-healing mechanism is the immune system of a human body. This biology-inspired idea has been used in many engineering designs but is rarely investigated in deep learning. This paper considers the post-training self-healing of a neural network, and proposes a closed-loop control formulation to automatically detect and fix the errors caused by various attacks or perturbations. We provide a margin-based analysis to explain how this formulation can improve the robustness of a classifier. To speed up the inference of the proposed self-healing network, we solve the control problem via improving the Pontryagin Maximum Principle-based solver. Lastly, we present an error estimation of the proposed framework for neural networks with nonlinear activation functions. We validate the performance on several network architectures against various perturbations. Since the self-healing method does not need a-priori information about data perturbations/attacks, it can handle a broad class of unforeseen perturbations.

==> Self-Healing Robust Neural Networks via Closed-Loop Control/introduction_original.tex <==
\section{Introduction}
Despite their success in massive engineering applications, deep neural networks are found to be vulnerable to perturbations of input data.
It has been shown that an imperceptible perturbation of an input image can cause misclassification in a well-trained neural network \citep{szegedy2013intriguing, goodfellow2014explaining}.
Even though deep neural networks have achieved state-of-the-art performance in many applications,
such as computer vision, natural language processing, the vulnerability of neural networks has raised security concerns in safety-critical applications. 

Many defense methods have been proposed to circumvent this issue,
and we summarize the existing methods into two main types: training-based defense which focuses on the classifier itself,
and data-based defense that exploits the underlying data information. 
Arguably, the most representative training-based defense is adversarial training \citep{madry2017towards, zhang2019theoretically, gowal2020uncovering} based on robust optimization.
This method successfully passed all adversarial attack evaluations in \cite{athalye2018obfuscated} and \cite{croce2020reliablef}.
However, such training-based methods have some limitations.
First, it requires retraining the model or training with an inner loop, which can be expensive for large-scale applications.
The requirement of training labels here can further pose security concerns.
Second, one often requires some information about the type of attacks anticipated, e.g. adversarial training simulates an attack using projected gradient ascent under a chosen norm, thus is adapted to such types of attacks.
Data-based defenses, such as reactive defense \citep{song2017pixeldefend, samangouei2018defense} and input transformation \citep{venugopalancountering},
are introduced as alternatives to training-based defenses in part to alleviate some of the aforementioned issues.
For example, input transformation can be applied without retraining the model, nor requiring label information.
However, there is limited understanding of the working principles behind these methods, and to date, they have not
been able to achieve the state of the art performance \citep{athalye2018obfuscated}.

In this paper,
\begin{itemize}[leftmargin=*]
    \item 
    we investigate the theoretical underpinnings of data-based defense methods through a margin-based analysis.
    We show that the adaptive process of data-based defenses is equivalent to a modification of the decision boundary, and hence the classifier margin.
    Based on this, we present a detailed margin-based analysis on the robustness of classification problems for data-based defenses.
    In particular, we introduce three types of margins that are of relevance, which involve an interplay of the ground truth classifier, the trained classifier and, the data manifold.
    We show that the performance of data-based defenses can be determined by these margins.
    \item
    Armed with this understanding, we consider a optimal control based hybrid defense scheme, the closed-loop control method \citep{chen2021towards}, that exploits both training and data-based defenses.
    The Pontryagin's Maximum Principle allows a efficient implementation of the closed-loop control framework,
    which enables its compatibility with both deep and wide neural networks.
    Since in the white-box setting, adversarial attacker has the control information and can utilize the control signals to further perturb the underlying model. 
    We apply control regularization on the applied controls.
    This consideration stabilizes the controlled dynamic by enforcing the control signals to explore low loss states in locally near regions.
    In particular, control regularization distinguishes the closed-loop control from conventional layer-wise projection.
    \item
    We provide an error analysis of the closed-loop control method in the most general form by considering nonlinear dynamic with nonlinear embedding manifolds.
    The theoretical setup aligns with our algorithm implementation without simplification. 
    \item
    We show the generalization by applying one set of controllers on various deep networks that belong to a same family.
    We empirically verify the effectiveness of closed-loop control against various adversarial attacks.
\end{itemize}

==> Self-Healing Robust Neural Networks via Closed-Loop Control/introduction_zz.tex <==
\section{Introduction}
Despite their success in massive engineering applications, deep neural networks are found to be vulnerable to perturbations of input data, fail to ensure fairness across sub-groups of data, and experience performance degradation when implemented on nano-scale integrated circuits with process variations. In order to ensure trustworthy AI, numerous techniques have been reported, including defense techniques such as adverserial training to improve robustness, fairness-aware training, and fault-tolerant hardware design. 

A fundamental question is: {\it can we design a self-healing process for neural networks}? 
In a figurative sense, self-healing properties can be ascribed to systems or processes, which by nature or design tend to correct any disturbances brought into them. 
For instance, in psychology, self healing often refers to the recovery of a patient from a psychological disturbance guided by instinct only. 
In semiconductor chip design, self healing means that an integrated circuit can automatically detect and fix the errors caused by imperfect nano-scale fabrication~\citep{sun2014indirect}. 
In the context of machine learning, a self-healing process of a neural network is expected to fix or mitigate some undesired issues by itself, either with or without a performance detector. 
We envision that self-healing techniques can be developed at different stages of AI model development and deployment, including data acquisition/preparation, model training, post-training tuning, and hardware implementation. 
The goal can be to improve the robustness, safety, fairness, privacy or their combinations. 

In this paper, we show that it is possible to build a self-healing neural network to achieve better robustness. 
It has been well known that an imperceptible perturbation of an input image can cause misclassification in a well-trained neural network \citep{szegedy2013intriguing, goodfellow2014explaining}. 
Many defense methods have been proposed to circumvent this issue,
and we summarize the existing methods into two main types: training-based defense which focuses on the classifier itself,
and data-based defense that exploits the underlying data information.
Arguably, the most representative training-based defense is adversarial training \citep{madry2017towards, zhang2019theoretically, gowal2020uncovering} based on robust optimization.
This method successfully passed all adversarial attack evaluations in \cite{athalye2018obfuscated} and \cite{croce2020reliablef}.
However, such training-based methods have some limitations.
First, it requires retraining the model or training with an inner loop, which can be expensive for large-scale applications.
Second, the requirement of modifying the underlying model can further degrade its performance when deployed for non-adversarial environments.
On the other hand, data-based defenses \citep{song2017pixeldefend, samangouei2018defense, venugopalancountering}
are introduced as alternatives to training-based defenses in part to alleviate some of the aforementioned issues.
This class of defense method can be applied without retraining the model.
However, there is limited understanding of the working principles behind these methods, and to date, they have not
been able to achieve the state of the art performance \citep{athalye2018obfuscated}.
In this paper, we investigate the theoretical underpinnings of data-based defense methods through a margin-based analysis.
Armed with this understanding,
we propose an optimal control formulation for the self-healing of a neural network and realize this proposal via the recent closed-loop control method \citep{chen2021towards}. 
The self-healing process via closed-loop control can be understood as a hybrid method as combining training-based and data-based methods.
As with data-based defenses, this method does not require retraining the model. Moreover, we can optionally use
label information, as in adversarial training, to gain higher performance.

\paragraph{Contribution Summary.} The specific contributions of this paper are summarized below:
\begin{itemize}[leftmargin=*]
    \item {\bf Closed-loop control formulation for post-training self-healing.} We consider a closed-loop control formulation \citep{chen2021towards} to achieve self healing in the post-training stage, with a goal to improve the robustness of a given neural network under a broad class of perturbations/attacks. This self-healing formulation has two key components: embedding functions at both input and hidden layers to detect the possible errors, and a control process to adjust the neurons of hidden layer to fix or mitigate these errors before making a prediction.

    \item {\bf Fast numerical solver for the closed-loop control.} The Pontryagin's Maximum Principle allows a efficient implementation of the closed-loop control framework,
    which enables its compatibility with both deep and wide neural networks.
    Since in the white-box setting, adversarial attacker has the control information and can utilize the applied controls to further perturb the underlying model. 
    We apply control regularization on the applied controls.
    This consideration stabilizes the controlled dynamic to explore low loss states in locally near regions.
    In particular, control regularization distinguishes the closed-loop control from conventional layer-wise projection.
    
    \item {\bf A margin-based analysis for data-based defense methods.}
    We investigate data-based defense methods through a margin-based analysis, and show
    that the adaptive process of data-based defenses is equivalent to a modification of the decision boundary and classifier margin.
    Based on this, we introduce three types of margins that are of relevance, which involve an interplay of the ground truth classifier, the trained classifier and, the data manifold.
    We show that the performance of data-based defenses can be determined by these margins.
    Furthermore, we analyze the behaviour of embedding function with a general nonlinear manifold.
    Armed with this understanding, we build embedding functions that exploit both model information and data structure.
    This leads to superior performance of the closed-loop control method.
    
    \item {\bf Theoretical Error Analysis.}
    We provide an error analysis of the closed-loop control method in the most general form by considering nonlinear dynamic with nonlinear embedding manifolds.
    The theoretical setup aligns with our algorithm implementation without simplification.
\end{itemize}

\paragraph{Additional notation}
Throughout this paper, we use $\lVert \mat{x} \rVert$ as a abbreviate of the $2$-norm of a vector $\mat{x}$, such that $\lVert \mat{x} \rVert = \sqrt{\sum_{i=1}^d \mat{x}_i^2}$.
For a third-order tensor $\mat{H} \in \mathbb{R}^d \times \mathbb{R}^d \times \mathbb{R}^d$,
we define a $2$-norm of $\mat{H}$ as $\lVert \mat{H} \rVert_{\ast} = \sqrt{ \sum_{i=1}^d \lVert \mat{H}_i \rVert^2 }$,
which is the $2$-norm of a vector where each element is the matrix $2$-norm of $\mat{H}_i$.
We abbreviate the Einstein notation as $\mat{H} (\mat{x}_1) (\mat{x}_2) \vcentcolon = \mat{H}_{i, j, k} \mat{x}_1^j \mat{x}_2^k$, and $\mat{H} (\mat{x}_1) (\mat{x}_2) \in \mathbb{R}^d$.

==> introduction_original.tex <==
\section{Introduction}
Despite their success in massive engineering applications, deep neural networks are found to be vulnerable to perturbations of input data.
It has been shown that an imperceptible perturbation of an input image can cause misclassification in a well-trained neural network \citep{szegedy2013intriguing, goodfellow2014explaining}.
Even though deep neural networks have achieved state-of-the-art performance in many applications,
such as computer vision, natural language processing, the vulnerability of neural networks has raised security concerns in safety-critical applications. 

Many defense methods have been proposed to circumvent this issue,
and we summarize the existing methods into two main types: training-based defense which focuses on the classifier itself,
and data-based defense that exploits the underlying data information. 
Arguably, the most representative training-based defense is adversarial training \citep{madry2017towards, zhang2019theoretically, gowal2020uncovering} based on robust optimization.
This method successfully passed all adversarial attack evaluations in \cite{athalye2018obfuscated} and \cite{croce2020reliablef}.
However, such training-based methods have some limitations.
First, it requires retraining the model or training with an inner loop, which can be expensive for large-scale applications.
The requirement of training labels here can further pose security concerns.
Second, one often requires some information about the type of attacks anticipated, e.g. adversarial training simulates an attack using projected gradient ascent under a chosen norm, thus is adapted to such types of attacks.
Data-based defenses, such as reactive defense \citep{song2017pixeldefend, samangouei2018defense} and input transformation \citep{venugopalancountering},
are introduced as alternatives to training-based defenses in part to alleviate some of the aforementioned issues.
For example, input transformation can be applied without retraining the model, nor requiring label information.
However, there is limited understanding of the working principles behind these methods, and to date, they have not
been able to achieve the state of the art performance \citep{athalye2018obfuscated}.

In this paper,
\begin{itemize}[leftmargin=*]
    \item 
    we investigate the theoretical underpinnings of data-based defense methods through a margin-based analysis.
    We show that the adaptive process of data-based defenses is equivalent to a modification of the decision boundary, and hence the classifier margin.
    Based on this, we present a detailed margin-based analysis on the robustness of classification problems for data-based defenses.
    In particular, we introduce three types of margins that are of relevance, which involve an interplay of the ground truth classifier, the trained classifier and, the data manifold.
    We show that the performance of data-based defenses can be determined by these margins.
    \item
    Armed with this understanding, we consider a optimal control based hybrid defense scheme, the closed-loop control method \citep{chen2021towards}, that exploits both training and data-based defenses.
    The Pontryagin's Maximum Principle allows a efficient implementation of the closed-loop control framework,
    which enables its compatibility with both deep and wide neural networks.
    Since in the white-box setting, adversarial attacker has the control information and can utilize the control signals to further perturb the underlying model. 
    We apply control regularization on the applied controls.
    This consideration stabilizes the controlled dynamic by enforcing the control signals to explore low loss states in locally near regions.
    In particular, control regularization distinguishes the closed-loop control from conventional layer-wise projection.
    \item
    We provide an error analysis of the closed-loop control method in the most general form by considering nonlinear dynamic with nonlinear embedding manifolds.
    The theoretical setup aligns with our algorithm implementation without simplification. 
    \item
    We show the generalization by applying one set of controllers on various deep networks that belong to a same family.
    We empirically verify the effectiveness of closed-loop control against various adversarial attacks.
\end{itemize}

==> introduction_zz.tex <==
\section{Introduction}
Despite their success in massive engineering applications, deep neural networks are found to be vulnerable to perturbations of input data, fail to ensure fairness across sub-groups of data, and experience performance degradation when implemented on nano-scale integrated circuits with process variations. In order to ensure trustworthy AI, numerous techniques have been reported, including defense techniques such as adverserial training to improve robustness, fairness-aware training, and fault-tolerant hardware design. 

A fundamental question is: {\it can we design a self-healing process for neural networks}? 
In a figurative sense, self-healing properties can be ascribed to systems or processes, which by nature or design tend to correct any disturbances brought into them. 
For instance, in psychology, self healing often refers to the recovery of a patient from a psychological disturbance guided by instinct only. 
In semiconductor chip design, self healing means that an integrated circuit can automatically detect and fix the errors caused by imperfect nano-scale fabrication~\citep{sun2014indirect}. 
In the context of machine learning, a self-healing process of a neural network is expected to fix or mitigate some undesired issues by itself, either with or without a performance detector. 
We envision that self-healing techniques can be developed at different stages of AI model development and deployment, including data acquisition/preparation, model training, post-training tuning, and hardware implementation. 
The goal can be to improve the robustness, safety, fairness, privacy or their combinations. 

In this paper, we show that it is possible to build a self-healing neural network to achieve better robustness. 
It has been well known that an imperceptible perturbation of an input image can cause misclassification in a well-trained neural network \citep{szegedy2013intriguing, goodfellow2014explaining}. 
Many defense methods have been proposed to circumvent this issue,
and we summarize the existing methods into two main types: training-based defense which focuses on the classifier itself,
and data-based defense that exploits the underlying data information.
Arguably, the most representative training-based defense is adversarial training \citep{madry2017towards, zhang2019theoretically, gowal2020uncovering} based on robust optimization.
This method successfully passed all adversarial attack evaluations in \cite{athalye2018obfuscated} and \cite{croce2020reliablef}.
However, such training-based methods have some limitations.
First, it requires retraining the model or training with an inner loop, which can be expensive for large-scale applications.
Second, the requirement of modifying the underlying model can further degrade its performance when deployed for non-adversarial environments.
On the other hand, data-based defenses \citep{song2017pixeldefend, samangouei2018defense, venugopalancountering}
are introduced as alternatives to training-based defenses in part to alleviate some of the aforementioned issues.
This class of defense method can be applied without retraining the model.
However, there is limited understanding of the working principles behind these methods, and to date, they have not
been able to achieve the state of the art performance \citep{athalye2018obfuscated}.
In this paper, we investigate the theoretical underpinnings of data-based defense methods through a margin-based analysis.
Armed with this understanding,
we propose an optimal control formulation for the self-healing of a neural network and realize this proposal via the recent closed-loop control method \citep{chen2021towards}. 
The self-healing process via closed-loop control can be understood as a hybrid method as combining training-based and data-based methods.
As with data-based defenses, this method does not require retraining the model. Moreover, we can optionally use
label information, as in adversarial training, to gain higher performance.

\paragraph{Contribution Summary.} The specific contributions of this paper are summarized below:
\begin{itemize}[leftmargin=*]
    \item {\bf Closed-loop control formulation for post-training self-healing.} We consider a closed-loop control formulation \citep{chen2021towards} to achieve self healing in the post-training stage, with a goal to improve the robustness of a given neural network under a broad class of perturbations/attacks. This self-healing formulation has two key components: embedding functions at both input and hidden layers to detect the possible errors, and a control process to adjust the neurons of hidden layer to fix or mitigate these errors before making a prediction.

    \item {\bf Fast numerical solver for the closed-loop control.} The Pontryagin's Maximum Principle allows a efficient implementation of the closed-loop control framework,
    which enables its compatibility with both deep and wide neural networks.
    Since in the white-box setting, adversarial attacker has the control information and can utilize the applied controls to further perturb the underlying model. 
    We apply control regularization on the applied controls.
    This consideration stabilizes the controlled dynamic to explore low loss states in locally near regions.
    In particular, control regularization distinguishes the closed-loop control from conventional layer-wise projection.
    
    \item {\bf A margin-based analysis for data-based defense methods.}
    We investigate data-based defense methods through a margin-based analysis, and show
    that the adaptive process of data-based defenses is equivalent to a modification of the decision boundary and classifier margin.
    Based on this, we introduce three types of margins that are of relevance, which involve an interplay of the ground truth classifier, the trained classifier and, the data manifold.
    We show that the performance of data-based defenses can be determined by these margins.
    Furthermore, we analyze the behaviour of embedding function with a general nonlinear manifold.
    Armed with this understanding, we build embedding functions that exploit both model information and data structure.
    This leads to superior performance of the closed-loop control method.
    
    \item {\bf Theoretical Error Analysis.}
    We provide an error analysis of the closed-loop control method in the most general form by considering nonlinear dynamic with nonlinear embedding manifolds.
    The theoretical setup aligns with our algorithm implementation without simplification.
\end{itemize}

\paragraph{Additional notation}
Throughout this paper, we use $\lVert \mat{x} \rVert$ as a abbreviate of the $2$-norm of a vector $\mat{x}$, such that $\lVert \mat{x} \rVert = \sqrt{\sum_{i=1}^d \mat{x}_i^2}$.
For a third-order tensor $\mat{H} \in \mathbb{R}^d \times \mathbb{R}^d \times \mathbb{R}^d$,
we define a $2$-norm of $\mat{H}$ as $\lVert \mat{H} \rVert_{\ast} = \sqrt{ \sum_{i=1}^d \lVert \mat{H}_i \rVert^2 }$,
which is the $2$-norm of a vector where each element is the matrix $2$-norm of $\mat{H}_i$.
We abbreviate the Einstein notation as $\mat{H} (\mat{x}_1) (\mat{x}_2) \vcentcolon = \mat{H}_{i, j, k} \mat{x}_1^j \mat{x}_2^k$, and $\mat{H} (\mat{x}_1) (\mat{x}_2) \in \mathbb{R}^d$.
